Formalization of Differential Privacy in Isabelle/HOL

Differential privacy is a statistical definition of privacy that has attracted the interest of both academia and industry. Its formulations are easy to understand, but the differential privacy of databases is complicated to determine. One of the reasons for this is that small changes in database programs can break their differential privacy. Therefore, formal verification of differential privacy has been studied for over a decade. In this paper, we propose an Isabelle/HOL library for formalizing differential privacy in a general setting. To our knowledge, it is the first formalization of differential privacy that supports continuous probability distributions. First, we formalize the standard definition of differential privacy and its basic properties. Second, we formalize the Laplace mechanism and its differential privacy. Finally, we formalize the differential privacy of the report noisy max mechanism.

==> rnm_old.tex <==
\section{Formalization of the Report Noisy Max Mechanism in Isabelle/HOL}
\label{sec:formal_RNM}
\begin{figure*}
\begin{isabelle}
\isacommand{lemma}\isamarkupfalse%
\ finer{\isacharunderscore}{\kern0pt}sensitivity{\isacharunderscore}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}xs{\isacharcomma}{\kern0pt}ys{\isacharparenright}{\kern0pt}\ {\isasymin}\ adj{\isacharunderscore}{\kern0pt}L{\isadigit{1}}{\isacharunderscore}{\kern0pt}norm{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query\ xs{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query\ ys{\isacharparenright}{\kern0pt}
\isanewline \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ {\isasymor}\ list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query\ ys{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query\ xs{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
%
\begin{isabelle}
\isacommand{lemma}\isamarkupfalse%
\ fst{\isacharunderscore}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax{\isacharunderscore}{\kern0pt}adj{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{fixes}\ xs\ ys\ rs\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list{\isachardoublequoteclose}\ \isakeyword{and}\ n\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ nat\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}length\ xs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}
\ \isakeyword{and}\ {\isachardoublequoteopen}length\ ys\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}
\ \isakeyword{and}\ {\isachardoublequoteopen}length\ rs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}
\ \isakeyword{and}\ adj{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ xs\ ys{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}fst\ {\isacharparenleft}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax\ {\isacharparenleft}{\kern0pt}map{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isacharplus}{\kern0pt}{\isacharparenright}{\kern0pt}\ xs\ rs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isasymge}\ {\isacharparenleft}{\kern0pt}fst\ {\isacharparenleft}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax\ {\isacharparenleft}{\kern0pt}map{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isacharplus}{\kern0pt}{\isacharparenright}{\kern0pt}\ ys\ rs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}
\isanewline \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  {\isasymand}\ {\isacharparenleft}{\kern0pt}fst\ {\isacharparenleft}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax\ {\isacharparenleft}{\kern0pt}map{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isacharplus}{\kern0pt}{\isacharparenright}{\kern0pt}\ xs\ rs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}fst\ {\isacharparenleft}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax\ {\isacharparenleft}{\kern0pt}map{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isacharplus}{\kern0pt}{\isacharparenright}{\kern0pt}\ ys\ rs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isachardoublequoteclose}
\end{isabelle}
%
\begin{isabelle}
\isacommand{lemma}\isamarkupfalse%
\ argmax{\isacharunderscore}{\kern0pt}insert{\isacharunderscore}{\kern0pt}i{\isacharunderscore}{\kern0pt}i{\isacharprime}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}m\ {\isasymle}\ n{\isachardoublequoteclose}\ \isakeyword{and}\ {\isachardoublequoteopen}length\ xs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}argmax{\isacharunderscore}{\kern0pt}insert\ k\ xs\ m\ {\isacharequal}{\kern0pt}\ m{\isacharparenright}{\kern0pt}\ {\isasymlongleftrightarrow}\ {\isacharparenleft}{\kern0pt}ereal\ k\ {\isasymge}\ {\isacharparenleft}{\kern0pt}fst\ {\isacharparenleft}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax\ xs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isasymand}\ {\isacharparenleft}{\kern0pt}ereal\ k\ {\isasymnoteq}\ {\isacharparenleft}{\kern0pt}fst\ {\isacharparenleft}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax\ {\isacharparenleft}{\kern0pt}drop\ m\ xs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
%
\begin{isabelle}
\isacommand{lemma}\isamarkupfalse%
\ DP{\isacharunderscore}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M{\isacharunderscore}{\kern0pt}i{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{fixes}\ xs\ ys\ rs\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list{\isachardoublequoteclose}\ \isakeyword{and}\ x\ y\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ real\ \isakeyword{and}\ i\ n\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ nat\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}length\ xs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\ \isakeyword{and}\ {\isachardoublequoteopen}length\ ys\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\ \isakeyword{and}\ {\isachardoublequoteopen}length\ rs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\isanewline
\ \ \ \ \isakeyword{and}\ adj{\isacharprime}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isachardoublequoteclose}\  \isakeyword{and}\ adj{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ xs\ ys{\isachardoublequoteclose}\ \isakeyword{and}\ {\isachardoublequoteopen}i\ {\isasymle}\ n{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ xs\ rs\ x\ i{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}exp\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ ys\ rs\ y\ i{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}
\isanewline \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  {\isasymand}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ ys\ rs\ y\ i{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}exp\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ xs\ rs\ x\ i{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
%
\begin{isabelle}
\isacommand{lemma}\isamarkupfalse%
\ DP{\isacharunderscore}{\kern0pt}RNM{\isacharprime}{\kern0pt}{\isacharunderscore}{\kern0pt}M{\isacharunderscore}{\kern0pt}i{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{fixes}\ xs\ ys\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list{\isachardoublequoteclose}\ \isakeyword{and}\ i\ n\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ nat\isanewline
\ \ \isakeyword{assumes}\ lxs{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}length\ xs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}
\ \isakeyword{and}\ lys{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}length\ ys\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}
\ \isakeyword{and}\ adj{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ xs\ ys{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ xs{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}exp\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ ys{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymand}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ ys{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}exp\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ xs{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
\caption{Formalizations of Lemmas \ref{lem:adjacent:counting_query}, \ref{lem:fst_max_argmax_adj}, \ref{lem:argmax_insert_i_i}, \ref{lem:DP_RNM_M_i} and \ref{DP_RNM'_M_i}.}\label{Fig:Lemmas_RNM}
\end{figure*}
In this section, we formalize the differential privacy of the report noisy max mechanism $\mathrm{RNM}_{\vec{q},m,\varepsilon}$, namely Propositions \ref{prop:DP:RNM_naive} and \ref{prop:DP:RNM_true}.
The report noisy max mechanism $\mathrm{RNM}_{\vec{q},m,\varepsilon}$ is implemented in Isabelle/HOL as follows:
\begin{isabelle}
\isacommand{definition}\isamarkupfalse%
\ RNM{\isacharunderscore}{\kern0pt}counting\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ {\isasymRightarrow}\ nat\ list\ {\isasymRightarrow}\ nat\ measure{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}RNM{\isacharunderscore}{\kern0pt}counting\ {\isasymepsilon}\ x\ {\isacharequal}{\kern0pt}\ do\ {\isacharbraceleft}{\kern0pt}\isanewline
\ y\ {\isasymleftarrow}\ Lap{\isacharunderscore}{\kern0pt}dist{\isacharunderscore}{\kern0pt}list\ {\isacharparenleft}{\kern0pt}{\isadigit{1}}\ {\isacharslash}{\kern0pt}\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query\ x{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\isanewline
\ return\ {\isacharparenleft}{\kern0pt}count{\isacharunderscore}{\kern0pt}space\ UNIV{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}argmax{\isacharunderscore}{\kern0pt}list\ y{\isacharparenright}{\kern0pt}\isanewline
\ {\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
Here, \isa{counting{\isacharunderscore}{\kern0pt}query} is an implementation of a tuple of counting queries;
\isa{argmax{\isacharunderscore}{\kern0pt}list} is an implementation of the mapping $(y_0,\ldots,y_{m-1}) \mapsto \argmax_{0\leq i < m} y_i$;
\isa{Lap{\isacharunderscore}{\kern0pt}dist{\isacharunderscore}{\kern0pt}list} is the procedure adding noise sampled from $\mathrm{Lap}(1/\varepsilon)$ given in Section \ref{sec:Lap_dist_list}.
We give formal proofs of its differential privacy.

\subsection{Argmax of lists}
We check the details of \isa{argmax{\isacharunderscore}{\kern0pt}list}, and formalize Lemmas \ref{lem:fst_max_argmax_adj} and \ref{lem:argmax_insert_i_i}.
First, we define the function \isa{max{\isacharunderscore}{\kern0pt}argmax} returning the pair of max and  argmax of a list\footnote{we assume that the maximum of the empty list is $-\infty$.}.
We then define \isa{argmax{\isacharunderscore}{\kern0pt}list} by taking the second components of pairs.
\begin{isabelle}
\isacommand{primrec}\isamarkupfalse%
\ max{\isacharunderscore}{\kern0pt}argmax\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list\ {\isasymRightarrow}\ {\isacharparenleft}{\kern0pt}ereal\ {\isasymtimes}\ nat{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}max{\isacharunderscore}{\kern0pt}argmax\ {\isacharbrackleft}{\kern0pt}{\isacharbrackright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isacharminus}{\kern0pt}{\isasyminfinity}{\isacharcomma}{\kern0pt}{\isadigit{0}}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}{\isacharbar}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}max{\isacharunderscore}{\kern0pt}argmax\ {\isacharparenleft}{\kern0pt}x{\isacharhash}{\kern0pt}xs{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}let\ {\isacharparenleft}{\kern0pt}m{\isacharcomma}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ max{\isacharunderscore}{\kern0pt}argmax\ xs\ in\ if\ x\ {\isachargreater}{\kern0pt}\ m\ then\ {\isacharparenleft}{\kern0pt}x{\isacharcomma}{\kern0pt}{\isadigit{0}}{\isacharparenright}{\kern0pt}\ else\ {\isacharparenleft}{\kern0pt}m{\isacharcomma}{\kern0pt}\ Suc\ i{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
\begin{isabelle}
\isacommand{definition}\isamarkupfalse%
\ argmax{\isacharunderscore}{\kern0pt}list\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}argmax{\isacharunderscore}{\kern0pt}list\ {\isacharequal}{\kern0pt}\ snd\ o\ max{\isacharunderscore}{\kern0pt}argmax\ {\isachardoublequoteclose}
\end{isabelle}
We then formalize Lemma \ref{lem:fst_max_argmax_adj} as \isa{fst{\isacharunderscore}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax{\isacharunderscore}{\kern0pt}adj} in Figure \ref{Fig:Lemmas_RNM}. 
Here,  \isa{fst\ {\isacharparenleft}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax ... {\isacharparenright}} is the maximum value of a list, and 
the premise \isa{adj} is corresponds to (A) in Lemma \ref{lem:adjacent:counting_query}.
%\isa{map{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isacharplus}{\kern0pt}{\isacharparenright}} is the operation taking the element-wise sum of lists. 

Next, we define the function that combining argmax and insertion of elements.
\begin{isabelle}
\isacommand{definition}\isamarkupfalse%
\ argmax{\isacharunderscore}{\kern0pt}insert\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ {\isasymRightarrow}\ real\ list\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}argmax{\isacharunderscore}{\kern0pt}insert\ k\ ks\ i\ {\isacharequal}{\kern0pt}\ argmax{\isacharunderscore}{\kern0pt}list\ {\isacharparenleft}{\kern0pt}list{\isacharunderscore}{\kern0pt}insert\ k\ ks\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
%\isacommand{definition}\isamarkupfalse%
%\ argmax{\isacharunderscore}{\kern0pt}insert\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ {\isasymRightarrow}\ real\ list\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
%\ \ {\isachardoublequoteopen}argmax{\isacharunderscore}{\kern0pt}insert\ k\ ks\ i\ {\isacharequal}{\kern0pt}\ argmax{\isacharunderscore}{\kern0pt}list\ {\isacharparenleft}{\kern0pt}list{\isacharunderscore}{\kern0pt}insert\ k\ ks\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
%\ \ {\isachardoublequoteopen}argmax{\isacharunderscore}{\kern0pt}insert\ k\ ks\ i\ {\isacharequal}{\kern0pt}\ argmax{\isacharunderscore}{\kern0pt}list\ {\isacharparenleft}{\kern0pt}take\ i\ ks\ {\isacharat}{\kern0pt}\ {\isacharbrackleft}{\kern0pt}k{\isacharbrackright}{\kern0pt}\ {\isacharat}{\kern0pt}\ drop\ i\ ks{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
Here, \isa{list{\isacharunderscore}{\kern0pt}insert\ k\ ks\ i = {\isacharparenleft}{\kern0pt}take\ i\ ks\ {\isacharat}{\kern0pt}\ {\isacharbrackleft}{\kern0pt}k{\isacharbrackright}{\kern0pt}\ {\isacharat}{\kern0pt}\ drop\ i\ ks{\isacharparenright}} 
is the list made by inserting the element \isa{k} to the list \isa{ks} at the \isa{i}-th position.
When \isa{k} and \isa{xs} correspond to $d_i$ and $\vec{d}_{- i}$ respectively, 
\isa{argmax{\isacharunderscore}{\kern0pt}insert\ k\ ks\ i} corresponds to ${\textstyle \argmax_{0 \leq j < m}} d_j$.
We then formalize Lemma \ref{lem:argmax_insert_i_i} as \isa{argmax{\isacharunderscore}{\kern0pt}insert{\isacharunderscore}{\kern0pt}i{\isacharunderscore}{\kern0pt}i{\isacharprime}} in Figure \ref{Fig:Lemmas_RNM}. 
%\begin{isabelle}
%\isacommand{lemma}\isamarkupfalse%
%\ argmax{\isacharunderscore}{\kern0pt}insert{\isacharunderscore}{\kern0pt}i{\isacharunderscore}{\kern0pt}i{\isacharprime}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
%\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}m\ {\isasymle}\ n{\isachardoublequoteclose}\ \isakeyword{and}\ {\isachardoublequoteopen}length\ xs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\isanewline
%\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}argmax{\isacharunderscore}{\kern0pt}insert\ k\ xs\ m\ {\isacharequal}{\kern0pt}\ m{\isacharparenright}{\kern0pt}\ {\isasymlongleftrightarrow}\ {\isacharparenleft}{\kern0pt}ereal\ k\ {\isasymge}\ {\isacharparenleft}{\kern0pt}fst\ {\isacharparenleft}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax\ xs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isasymand}\ {\isacharparenleft}{\kern0pt}ereal\ k\ {\isasymnoteq}\ {\isacharparenleft}{\kern0pt}fst\ {\isacharparenleft}{\kern0pt}max{\isacharunderscore}{\kern0pt}argmax\ {\isacharparenleft}{\kern0pt}drop\ m\ xs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
%\end{isabelle}

\subsection{Differential Privacy of the main body}
We prove the differential privacy of $\mathrm{RNM'}_{m,\varepsilon} \circ c$ for general $X$, $R^{\mathrm{adj}}$ and $c \colon X \to \Real^m$
satisfying similar statement as Lemma \ref{lem:adjacent:counting_query} (intuitively ``(A) or (B) holds'').
Later, we instantiate them as expected.
For proof, we introduce the following locale.
\begin{isabelle}
\isacommand{locale}\isamarkupfalse%
\ Lap{\isacharunderscore}{\kern0pt}Mechanism{\isacharunderscore}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}mainpart\ {\isacharequal}{\kern0pt}\isanewline
\ \ \isakeyword{fixes}\ M{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}{\isachardoublequoteopen}{\isacharprime}{\kern0pt}a\ measure{\isachardoublequoteclose}\isanewline
\ \ \ \ \isakeyword{and}\ adj{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}{\isachardoublequoteopen}{\isacharprime}{\kern0pt}a\ rel{\isachardoublequoteclose}\isanewline
\ \ \ \ \isakeyword{and}\ c{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}{\isachardoublequoteopen}{\isacharprime}{\kern0pt}a\ {\isasymRightarrow}\ real\ list{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{assumes}\ c{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}c\ {\isasymin}\ M\ {\isasymrightarrow}\isactrlsub M\ {\isacharparenleft}{\kern0pt}listM\ borel{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isakeyword{and}\ cond{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isasymforall}\ {\isacharparenleft}{\kern0pt}x{\isacharcomma}{\kern0pt}y{\isacharparenright}{\kern0pt}\ {\isasymin}\ adj{\isachardot}{\kern0pt}\ list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}x\ y{\isachardot}{\kern0pt}\ y\ {\isasymle}\ x\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}c\ x{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}c\ y{\isacharparenright}{\kern0pt}\ {\isasymor}\ list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}x\ y{\isachardot}{\kern0pt}\ y\ {\isasymle}\ x\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}c\ y{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}c\ x{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \ \ \isakeyword{and}\ adj{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}adj\ {\isasymsubseteq}\ {\isacharparenleft}{\kern0pt}space\ M{\isacharparenright}{\kern0pt}\ {\isasymtimes}\ {\isacharparenleft}{\kern0pt}space\ M{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\isakeyword{begin}
\end{isabelle}
%
\begin{isabelle}
\isacommand{definition}\isamarkupfalse%
\ LapMech{\isacharunderscore}{\kern0pt}RNM\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ {\isasymRightarrow}\ {\isacharprime}{\kern0pt}a\ {\isasymRightarrow}\ nat\ measure{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}LapMech{\isacharunderscore}{\kern0pt}RNM\ {\isasymepsilon}\ x\ {\isacharequal}{\kern0pt}\ do\ {\isacharbraceleft}{\kern0pt}y\ {\isasymleftarrow}\ Lap{\isacharunderscore}{\kern0pt}dist{\isacharunderscore}{\kern0pt}list\ {\isacharparenleft}{\kern0pt}{\isadigit{1}}\ {\isacharslash}{\kern0pt}\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}c\ x{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\ return\ {\isacharparenleft}{\kern0pt}count{\isacharunderscore}{\kern0pt}space\ UNIV{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}argmax{\isacharunderscore}{\kern0pt}list\ y{\isacharparenright}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
%
%\begin{isabelle}
%\isacommand{lemma}\isamarkupfalse%
%\ measurable{\isacharunderscore}{\kern0pt}LapMech{\isacharunderscore}{\kern0pt}RNM{\isacharbrackleft}{\kern0pt}measurable{\isacharbrackright}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
%\ \ \isakeyword{shows}\ {\isachardoublequoteopen}LapMech{\isacharunderscore}{\kern0pt}RNM\ {\isasymepsilon}\ {\isasymin}\ M\ {\isasymrightarrow}\isactrlsub M\ prob{\isacharunderscore}{\kern0pt}algebra{\isacharparenleft}{\kern0pt}count{\isacharunderscore}{\kern0pt}space\ UNIV{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
%\end{isabelle}

We formalize Lemmas \ref{lem:DP_RNM_M_i} and \ref{DP_RNM'_M_i}, and
prove the differential privacy of \isa{LapMech{\isacharunderscore}{\kern0pt}RNM}. 
We set the following context, and focus on the main body \isa{RNM{\isacharprime}}.

\begin{isabelle}
\isacommand{context}\isamarkupfalse%
\isanewline
\ \ \isakeyword{fixes}\ {\isasymepsilon}{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}real
\isanewline
\ \ \isakeyword{assumes}\ pose{\isacharcolon}{\kern0pt}{\isachardoublequoteopen}{\isadigit{0}}\ {\isacharless}{\kern0pt}\ {\isasymepsilon}{\isachardoublequoteclose}\isanewline
\isakeyword{begin}%
\end{isabelle}
%\tetsuya{TODO: rebuild the definition of RNM'}
\begin{isabelle}
\isacommand{definition}\isamarkupfalse%
\ RNM{\isacharprime}{\kern0pt}\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list\ {\isasymRightarrow}\ nat\ measure{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}RNM{\isacharprime}{\kern0pt}\ zs\ {\isacharequal}{\kern0pt}\ do\ {\isacharbraceleft}{\kern0pt}y\ {\isasymleftarrow}\ Lap{\isacharunderscore}{\kern0pt}dist{\isacharunderscore}{\kern0pt}list\ {\isacharparenleft}{\kern0pt}{\isadigit{1}}\ {\isacharslash}{\kern0pt}\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}zs{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\ return\ {\isacharparenleft}{\kern0pt}count{\isacharunderscore}{\kern0pt}space\ UNIV{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}argmax{\isacharunderscore}{\kern0pt}list\ y{\isacharparenright}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}

%\begin{isabelle}
%\isacommand{lemma}\isamarkupfalse%
%\ measurable{\isacharunderscore}{\kern0pt}RNM{\isacharprime}{\kern0pt}{\isacharbrackleft}{\kern0pt}measurable{\isacharbrackright}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
%\ \ \isakeyword{shows}\ {\isachardoublequoteopen}RNM{\isacharprime}{\kern0pt}\ {\isasymin}\ listM\ borel\ {\isasymrightarrow}\isactrlsub M\ prob{\isacharunderscore}{\kern0pt}algebra{\isacharparenleft}{\kern0pt}count{\isacharunderscore}{\kern0pt}space\ UNIV{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
%\end{isabelle}

We formalize $p_i$ (see equation (\ref{eq:p_i})) as follows:
\begin{isabelle}
\isacommand{definition}\isamarkupfalse%
\ RNM{\isacharunderscore}{\kern0pt}M\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list\ {\isasymRightarrow}\ real\ list\ {\isasymRightarrow}\ real\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ nat\ measure{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}RNM{\isacharunderscore}{\kern0pt}M\ cs\ rs\ d\ i\ {\isacharequal}{\kern0pt}\ do{\isacharbraceleft}{\kern0pt}r\ {\isasymleftarrow}\ {\isacharparenleft}{\kern0pt}Lap{\isacharunderscore}{\kern0pt}dist{\isadigit{0}}\ {\isacharparenleft}{\kern0pt}{\isadigit{1}}{\isacharslash}{\kern0pt}{\isasymepsilon}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\ return\ {\isacharparenleft}{\kern0pt}count{\isacharunderscore}{\kern0pt}space\ UNIV{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}argmax{\isacharunderscore}{\kern0pt}insert\ {\isacharparenleft}{\kern0pt}r{\isacharplus}{\kern0pt}d{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}{\isacharparenleft}{\kern0pt}{\isasymlambda}\ {\isacharparenleft}{\kern0pt}xs{\isacharcomma}{\kern0pt}ys{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ {\isacharparenleft}{\kern0pt}map{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isacharplus}{\kern0pt}{\isacharparenright}{\kern0pt}\ xs\ ys{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharparenleft}{\kern0pt}cs{\isacharcomma}{\kern0pt}\ rs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ i{\isacharparenright}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
We here relate variables \isa{r}, \isa{d}, \isa{rs} and \isa{cs} with
$r_i$, $c_i$, $\vec{r}_{- i}$ and $\vec{c}_{- i}$ respectively.
Then, \isa{RNM{\isacharunderscore}{\kern0pt}M\ cs\ rs\ d\ i} is an implementation of
the following probability distribution:
\[
\{r_i \leftarrow \mathrm{Lap}(1/\varepsilon);\return {\textstyle \argmax_{0 \leq j < m}} (c_j + r_j) \} \in \prob(\Nat).
\]
Then, $p_i$ is implemented as \isa{{\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ xs\ rs\ x\ i{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}}.
We then formalize Lemma \ref{lem:DP_RNM_M_i}  as \isa{DP{\isacharunderscore}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M{\isacharunderscore}{\kern0pt}i} in Figure \ref{Fig:Lemmas_RNM}.
%\begin{isabelle}
%\isacommand{lemma}\isamarkupfalse%
%\ DP{\isacharunderscore}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M{\isacharunderscore}{\kern0pt}i{\isacharcolon}{\kern0pt}\isanewline
%\ \ \isakeyword{fixes}\ xs\ ys\ rs\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list{\isachardoublequoteclose}\ \isakeyword{and}\ x\ y\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ real\ \isakeyword{and}\ i\ n\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ nat\isanewline
%\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}length\ xs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\ \isakeyword{and}\ {\isachardoublequoteopen}length\ ys\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\ \isakeyword{and}\ {\isachardoublequoteopen}length\ rs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\isanewline
%\ \ \ \ \isakeyword{and}\ adj{\isacharprime}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isachardoublequoteclose}\isanewline
%\ \ \ \ \isakeyword{and}\ adj{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ xs\ ys{\isachardoublequoteclose}\ \isakeyword{and}\ {\isachardoublequoteopen}i\ {\isasymle}\ n{\isachardoublequoteclose}\isanewline
%\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ xs\ rs\ x\ i{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}exp\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ ys\ rs\ y\ i{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymand}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ ys\ rs\ y\ i{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}exp\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ xs\ rs\ x\ i{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
%\end{isabelle}

Next, we formalize Lemma \ref{DP_RNM'_M_i} as \isa{DP{\isacharunderscore}{\kern0pt}RNM{\isacharprime}{\kern0pt}{\isacharunderscore}{\kern0pt}M{\isacharunderscore}{\kern0pt}i} in Figure \ref{Fig:Lemmas_RNM}.
If $1 < m$, we formalize equation (\ref{eq:RNM_expand}):
%\begin{isabelle}
%\isacommand{lemma}\isamarkupfalse%
%\ DP{\isacharunderscore}{\kern0pt}RNM{\isacharprime}{\kern0pt}{\isacharunderscore}{\kern0pt}M{\isacharunderscore}{\kern0pt}i{\isacharcolon}{\kern0pt}\isanewline
%\ \ \isakeyword{fixes}\ xs\ ys\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list{\isachardoublequoteclose}\ \isakeyword{and}\ i\ n\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ nat\isanewline
%\ \ \isakeyword{assumes}\ lxs{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}length\ xs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\isanewline
%\ \ \ \ \isakeyword{and}\ lys{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}length\ ys\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\isanewline
%\ \ \ \ \isakeyword{and}\ adj{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ xs\ ys{\isachardoublequoteclose}\isanewline
%\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ xs{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}exp\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ ys{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymand}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ ys{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}\ {\isasymle}\ {\isacharparenleft}{\kern0pt}exp\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharasterisk}{\kern0pt}\ {\isasymP}{\isacharparenleft}{\kern0pt}j\ in\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ xs{\isacharparenright}{\kern0pt}{\isachardot}{\kern0pt}\ j\ {\isacharequal}{\kern0pt}\ i{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
%\end{isabelle}
%
%The formal proof is done .
%The following lemma is important: 
%
\begin{isabelle}
\isacommand{lemma}\isamarkupfalse%
\ RNM{\isacharprime}{\kern0pt}{\isacharunderscore}{\kern0pt}expand{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{fixes}\ n\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ nat\isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}length\ xs\ {\isacharequal}{\kern0pt}\ n{\isachardoublequoteclose}\ \isakeyword{and}\ {\isachardoublequoteopen}i\ {\isasymle}\ n{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ {\isacharparenleft}{\kern0pt}list{\isacharunderscore}{\kern0pt}insert\ x\ xs\ i{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isacharequal}{\kern0pt}\ do{\isacharbraceleft}{\kern0pt}rs\ {\isasymleftarrow}\ {\isacharparenleft}{\kern0pt}Lap{\isacharunderscore}{\kern0pt}dist{\isadigit{0}}{\isacharunderscore}{\kern0pt}list\ {\isacharparenleft}{\kern0pt}{\isadigit{1}}\ {\isacharslash}{\kern0pt}\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}length\ xs{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isacharsemicolon}{\kern0pt}\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}M\ xs\ rs\ x\ i{\isacharparenright}{\kern0pt}{\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}
If $m = 0,1$, we show \isa{RNM' xs = return (count\_space UNIV) 0} directly.
For such corner cases,  we need to give extra lemmas.

Finally, we conclude the ``differential privacy'' of the main body $ \mathrm{RNM'}_{m,\varepsilon}$.
We temporally use an asymmetric relation corresponding to (A) in Lemma \ref{lem:adjacent:counting_query}.
\begin{isabelle}
%\isacommand{lemma}\isamarkupfalse%
%\ DP{\isacharunderscore}{\kern0pt}divergence{\isacharunderscore}{\kern0pt}RNM{\isacharprime}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
%\ \ \isakeyword{fixes}\ xs\ ys\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}real\ list{\isachardoublequoteclose}\isanewline
%\ \ \isakeyword{assumes}\ adj{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ xs\ ys{\isachardoublequoteclose}\isanewline
%\ \ \isakeyword{shows}\ {\isachardoublequoteopen}DP{\isacharunderscore}{\kern0pt}divergence\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ xs{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ ys{\isacharparenright}{\kern0pt}\ {\isasymepsilon}\ {\isasymle}\ {\isadigit{0}}\ {\isasymand}\ DP{\isacharunderscore}{\kern0pt}divergence\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ ys{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}RNM{\isacharprime}{\kern0pt}\ xs{\isacharparenright}{\kern0pt}\ {\isasymepsilon}\ {\isasymle}\ {\isadigit{0}}{\isachardoublequoteclose}
\isacommand{lemma}\isamarkupfalse%
\ differential{\isacharunderscore}{\kern0pt}privacy{\isacharunderscore}{\kern0pt}LapMech{\isacharunderscore}{\kern0pt}RNM{\isacharprime}{\kern0pt}{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}differential{\isacharunderscore}{\kern0pt}privacy\ RNM{\isacharprime}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharparenleft}{\kern0pt}xs{\isacharcomma}{\kern0pt}\ ys{\isacharparenright}{\kern0pt}\ {\isacharbar}{\kern0pt}\ xs\ ys{\isachardot}{\kern0pt}\ list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ xs\ ys\ {\isacharbraceright}{\kern0pt}\ {\isasymepsilon}\ {\isadigit{0}}{\isachardoublequoteclose}
\end{isabelle}
%By the symmetry between conditions (A) and (B), we obtain 
%\begin{isabelle}
%\isacommand{corollary}\isamarkupfalse%
%\ differential{\isacharunderscore}{\kern0pt}privacy{\isacharunderscore}{\kern0pt}LapMech{\isacharunderscore}{\kern0pt}RNM{\isacharprime}{\kern0pt}{\isacharunderscore}{\kern0pt}sym{\isacharcolon}{\kern0pt}\isanewline
%\ \ \isakeyword{shows}\ {\isachardoublequoteopen}differential{\isacharunderscore}{\kern0pt}privacy\ RNM{\isacharprime}{\kern0pt}\ {\isacharbraceleft}{\kern0pt}{\isacharparenleft}{\kern0pt}xs{\isacharcomma}{\kern0pt}\ ys{\isacharparenright}{\kern0pt}\ {\isacharbar}{\kern0pt}\ xs\ ys{\isachardot}{\kern0pt}\ list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ xs\ ys\ {\isasymor}\ list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ ys\ xs\ {\isacharbraceright}{\kern0pt}\ {\isasymepsilon}\ {\isadigit{0}}{\isachardoublequoteclose}
%\end{isabelle}
From the symmetry between conditions (A) and (B), that asymmetric relation can be extended to the symmetric relation corresponding to ``(A) or (B) holds''.
Then, by the assumption on \isa{c} and \isa{differential{\isacharunderscore}{\kern0pt}privacy{\isacharunderscore}{\kern0pt}preprocessing}, 
we conclude the differential privacy of \isa{LapMech{\isacharunderscore}{\kern0pt}RNM}.
\begin{isabelle}
\isacommand{theorem}\isamarkupfalse%
\ differential{\isacharunderscore}{\kern0pt}privacy{\isacharunderscore}{\kern0pt}LapMech{\isacharunderscore}{\kern0pt}RNM{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}differential{\isacharunderscore}{\kern0pt}privacy\ {\isacharparenleft}{\kern0pt}LapMech{\isacharunderscore}{\kern0pt}RNM\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ adj\ {\isasymepsilon}\ {\isadigit{0}}{\isachardoublequoteclose}
\end{isabelle}

\subsection{Instantiation of  counting queries}
We here check the details of \isa{counting{\isacharunderscore}{\kern0pt}query} to formalize Propositions \ref{prop:DP:RNM_naive} and \ref{prop:DP:RNM_naive}.
We introduce the following locale to implement a tuple $\vec{q} \colon \Nat^{|\mathcal{X}|} \to \Nat^m$ of counting queries.
\begin{isabelle}
\isacommand{locale}\isamarkupfalse%
\ Lap{\isacharunderscore}{\kern0pt}Mechanism{\isacharunderscore}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}counting\ {\isacharequal}{\kern0pt}\isanewline
\ \ \isakeyword{fixes}\ n{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}nat\ \isakeyword{and}\ m{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}nat\ \isakeyword{and}\ Q\ {\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}nat\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ bool{\isachardoublequoteclose}\ \isanewline
\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}{\isasymAnd}i{\isachardot}{\kern0pt}\ i\ {\isasymin}\ {\isacharbraceleft}{\kern0pt}{\isadigit{0}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isacharless}{\kern0pt}m{\isacharbraceright}{\kern0pt}\ {\isasymLongrightarrow}\ {\isacharparenleft}{\kern0pt}Q\ i{\isacharparenright}{\kern0pt}\ {\isasymin}\ UNIV\ {\isasymrightarrow}\ UNIV{\isachardoublequoteclose}\isanewline
\isakeyword{begin}
\end{isabelle}
Here \isa{n} is the number $|\mathcal{X}|$ of data types, and \isa{m} is the number of counting queries.
Each \isa{Q i} is a predicate corresponding to a subset $\mathcal{X}_{q_i}$ of types which counting query $q_i$ counts.  
The assumption is for the totality of each \isa{Q i}.
We also interpret locales \isa{L{\isadigit{1}}{\isacharunderscore}{\kern0pt}norm{\isacharunderscore}{\kern0pt}list} 
and \isa{results{\isacharunderscore}{\kern0pt}AFDP} to instantiate $\Nat^{|\mathcal{X}|}$, adjacency of datasets, and to recall basic results of DP. 
%\begin{isabelle}
%\isacommand{interpretation}\isamarkupfalse%
%\ L{\isadigit{1}}{\isacharunderscore}{\kern0pt}norm{\isacharunderscore}{\kern0pt}list\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}UNIV{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}nat\ set{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}{\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ {\isasymbar}int\ x\ {\isacharminus}{\kern0pt}\ int\ y{\isasymbar}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}n
%\end{isabelle}

We then implement each counting query $q_i \colon \Nat^\mathcal{X} \to \Nat$.
\begin{isabelle}
\isacommand{primrec}\isamarkupfalse%
\ counting{\isacharprime}{\kern0pt}{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}{\isachardoublequoteopen}nat\ {\isasymRightarrow}\ nat\ {\isasymRightarrow}\ nat\ list\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}counting{\isacharprime}{\kern0pt}\ i\ {\isadigit{0}}\ {\isacharunderscore}{\kern0pt}\ {\isacharequal}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\ {\isacharbar}{\kern0pt}\isanewline
\ \ {\isachardoublequoteopen}counting{\isacharprime}{\kern0pt}\ i\ {\isacharparenleft}{\kern0pt}Suc\ k{\isacharparenright}{\kern0pt}\ xs\ {\isacharequal}{\kern0pt}\ {\isacharparenleft}{\kern0pt}if\ Q\ i\ k\ then\ {\isacharparenleft}{\kern0pt}nth{\isacharunderscore}{\kern0pt}total\ {\isadigit{0}}\ xs\ k{\isacharparenright}{\kern0pt}\ else\ {\isadigit{0}}{\isacharparenright}{\kern0pt}\ {\isacharplus}{\kern0pt}\ counting{\isacharprime}{\kern0pt}\ i\ k\ xs{\isachardoublequoteclose}
\end{isabelle}
%
\begin{isabelle}
\isacommand{definition}\isamarkupfalse%
\ counting{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}{\isachardoublequoteopen}nat\ {\isasymRightarrow}\ nat\ list\ {\isasymRightarrow}\ nat{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}counting\ i\ xs\ {\isacharequal}{\kern0pt}\ counting{\isacharprime}{\kern0pt}\ i\ {\isacharparenleft}{\kern0pt}length\ xs{\isacharparenright}{\kern0pt}\ xs{\isachardoublequoteclose}
\end{isabelle}
Here, each counting query $q_k$ is implemented as  \isa{counting k}. 
The function \isa{nth{\isacharunderscore}{\kern0pt}total} is a totalized version of Isabelle/HOL's \isa{nth}, which is more convenient for measurability proofs.

We then implement the tuple $ \vec{q} = (q_0,\ldots,q_{m-1})$ as:
\begin{isabelle}
\isacommand{definition}\isamarkupfalse%
\ counting{\isacharunderscore}{\kern0pt}query{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}{\isachardoublequoteopen}nat\ list\ {\isasymRightarrow}\ nat\ list{\isachardoublequoteclose}\ \isakeyword{where}\isanewline
\ \ {\isachardoublequoteopen}counting{\isacharunderscore}{\kern0pt}query\ xs\ {\isacharequal}{\kern0pt}\ map\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ k{\isachardot}{\kern0pt}\ counting\ k\ xs{\isacharparenright}{\kern0pt}\ {\isacharbrackleft}{\kern0pt}{\isadigit{0}}{\isachardot}{\kern0pt}{\isachardot}{\kern0pt}{\isacharless}{\kern0pt}m{\isacharbrackright}{\kern0pt}{\isachardoublequoteclose}
\end{isabelle}

\subsubsection{Naive evaluation}
We formalize Proposition \ref{prop:DP:RNM_naive}.
We define the sensitivity of \isa{counting{\isacharunderscore}{\kern0pt}query} using the locale \isa{Lap{\isacharunderscore}{\kern0pt}Mechanism{\isacharunderscore}{\kern0pt}list}.
\begin{isabelle}
\isacommand{interpretation}\isamarkupfalse%
\ Lap{\isacharunderscore}{\kern0pt}Mechanism{\isacharunderscore}{\kern0pt}list\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}listM\ {\isacharparenleft}{\kern0pt}count{\isacharunderscore}{\kern0pt}space\ UNIV{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}\ {\isachardoublequoteopen}counting{\isacharunderscore}{\kern0pt}query{\isachardoublequoteclose}\ {\isachardoublequoteopen}adj{\isacharunderscore}{\kern0pt}L{\isadigit{1}}{\isacharunderscore}{\kern0pt}norm{\isachardoublequoteclose}\ m
\end{isabelle}
We then check the sensitivity of \isa{counting{\isacharunderscore}{\kern0pt}query}:
\begin{isabelle}
\isacommand{lemma}\isamarkupfalse%
\ sensitvity{\isacharunderscore}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}sensitivity\ {\isasymle}\ m{\isachardoublequoteclose}
\end{isabelle}
Finally, by applying \isa{DP{\isacharunderscore}{\kern0pt}Lap{\isacharunderscore}{\kern0pt}dist{\isacharunderscore}{\kern0pt}list} and the basic properties of differential privacy (formalized in Isabelle/HOL),
we conclude the following formal version of Proposition \ref{prop:DP:RNM_naive}:
\begin{isabelle}
\isacommand{theorem}\isamarkupfalse%
\ Naive{\isacharunderscore}{\kern0pt}differential{\isacharunderscore}{\kern0pt}privacy{\isacharunderscore}{\kern0pt}LapMech{\isacharunderscore}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}AFDP{\isacharcolon}{\kern0pt}\isanewline
\isakeyword{assumes}\ pose{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymepsilon}{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}real{\isacharparenright}{\kern0pt}\ {\isachargreater}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
\isakeyword{shows}\ {\isachardoublequoteopen}differential{\isacharunderscore}{\kern0pt}privacy{\isacharunderscore}{\kern0pt}AFDP\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}counting\ {\isasymepsilon}{\isacharparenright}{\kern0pt}{\isacharparenleft}{\kern0pt}real\ {\isacharparenleft}{\kern0pt}m\ {\isacharasterisk}{\kern0pt}\ {\isasymepsilon}{\isacharparenright}{\kern0pt}{\isacharparenright}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}
\end{isabelle}

\subsubsection{Finar evaluation}
We formalize Proposition \ref{prop:DP:RNM_true}.
It suffices to interpret the locale \isa{Lap{\isacharunderscore}{\kern0pt}Mechanism{\isacharunderscore}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}mainpart} with \isa{counting{\isacharunderscore}{\kern0pt}query}. 
%We instantiate $X = \Nat^{|\mathcal{X}|}$, $R^\mathrm{adj} = \{ (D,D') ~|~ \|D  - D' \|  \leq 1\}$ and $c = \vec{q}$ to the proof of differential privacy of $\mathrm{RNM'}_{m,\varepsilon} \circ c$.
%We go back to the locale \isa{ Lap{\isacharunderscore}{\kern0pt}Mechanism{\isacharunderscore}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}counting},
%and prove the differential privacy of \isa{RNM{\isacharunderscore}{\kern0pt}counting}.
The remaining task is formalizing Lemma \ref{lem:adjacent:counting_query}.
It is given as \isa{ finer{\isacharunderscore}{\kern0pt}sensitivity{\isacharunderscore}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query} in Figure \ref{Fig:Lemmas_RNM}.

%\begin{isabelle}
%\isacommand{lemma}\isamarkupfalse%
%\ finer{\isacharunderscore}{\kern0pt}sensitivity{\isacharunderscore}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query{\isacharcolon}{\kern0pt}\isanewline
%\ \ \isakeyword{assumes}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}xs{\isacharcomma}{\kern0pt}ys{\isacharparenright}{\kern0pt}\ {\isasymin}\ adj{\isacharunderscore}{\kern0pt}L{\isadigit{1}}{\isacharunderscore}{\kern0pt}norm{\isachardoublequoteclose}\isanewline
%\ \ \isakeyword{shows}\ {\isachardoublequoteopen}list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query\ xs{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query\ ys{\isacharparenright}{\kern0pt}\ {\isasymor}\ list{\isacharunderscore}{\kern0pt}all{\isadigit{2}}\ {\isacharparenleft}{\kern0pt}{\isasymlambda}\ x\ y{\isachardot}{\kern0pt}\ x\ {\isasymge}\ y\ {\isasymand}\ x\ {\isasymle}\ y\ {\isacharplus}{\kern0pt}\ {\isadigit{1}}{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query\ ys{\isacharparenright}{\kern0pt}\ {\isacharparenleft}{\kern0pt}counting{\isacharunderscore}{\kern0pt}query\ xs{\isacharparenright}{\kern0pt}{\isachardoublequoteclose}
%\end{isabelle}
Combining the proofs on the main body, we conclude the formal version of Proposition \ref{prop:DP:RNM_true}:
\begin{isabelle}
\isacommand{theorem}\isamarkupfalse%
\ differential{\isacharunderscore}{\kern0pt}privacy{\isacharunderscore}{\kern0pt}LapMech{\isacharunderscore}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}AFDP{\isacharcolon}{\kern0pt}\isanewline
\ \ \isakeyword{assumes}\ pose{\isacharcolon}{\kern0pt}\ {\isachardoublequoteopen}{\isacharparenleft}{\kern0pt}{\isasymepsilon}{\isacharcolon}{\kern0pt}{\isacharcolon}{\kern0pt}real{\isacharparenright}{\kern0pt}\ {\isachargreater}{\kern0pt}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{shows}\ {\isachardoublequoteopen}differential{\isacharunderscore}{\kern0pt}privacy{\isacharunderscore}{\kern0pt}AFDP\ {\isacharparenleft}{\kern0pt}RNM{\isacharunderscore}{\kern0pt}counting\ {\isasymepsilon}{\isacharparenright}{\kern0pt}\ {\isasymepsilon}\ {\isadigit{0}}{\isachardoublequoteclose}
\end{isabelle}
